How to Agree to Disagree: Managing Ontological Perspectives using Standpoint Logic

The importance of taking individual, potentially conflicting perspectives into account when dealing with knowledge has been widely recognised. Many existing ontology management approaches fully merge knowledge perspectives, which may require weakening in order to maintain consistency; others represent the distinct views in an entirely detached way. As an alternative, we propose Standpoint Logic, a simple, yet versatile multi-modal logic "add-on" for existing KR languages intended for the integrated representation of domain knowledge relative to diverse, possibly conflicting standpoints, which can be hierarchically organised, combined and put in relation to each other. Starting from the generic framework of First-Order Standpoint Logic (FOSL), we subsequently focus our attention on the fragment of sentential formulas, for which we provide a polytime translation into the standpoint-free version. This result yields decidability and favourable complexities for a variety of highly expressive decidable fragments of first-order logic. Using some elaborate encoding tricks, we then establish a similar translation for the very expressive description logic SROIQb_s underlying the OWL 2 DL ontology language. By virtue of this result, existing highly optimised OWL reasoners can be used to provide practical reasoning support for ontology languages extended by standpoint modelling.

==> sections/Introduction.tex <==


%%%%%% DRAGON

-In knowledge integration is challenging, among other reasons because semantic heterogeneity is pervasive.

Knowledge bases encode different points of view, modelisations of a domain, granularity, ...

--Example 1

-In the global scale, unification is difficult because diversity is beneficial: we want to have good models for out task... but we also want them to interoperate.

--Example 2

%%%%%% SWORD

In CITE, we outlined a formalism aligned with philisophical theories of language and with pleasant computational properties for the propositional case. This was however insuficient for most applied scenarios where more expressivity was needed. In this paper, we go a step further. We propose a first-order framework. We explore the expressivity with an example. We select a fragment and .... We transfer this to the fragment of SROIQ, for which a transformation is also provided

%%%%%% TREASURE

With this, we gain a tool with which we can preserve different perspectives, integrated in a system, not only with good computational properties but with the capacity to reuse existing off-the-shelf reasoners.



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


Due to the availability on the Internet of a wide variety of
soures of information on losely related topis, the problem of providing
seamless, integrated access to such sources has become (again) a major
researh challenge. Although this problem has been studied for several
deades, espeially in the database ommunity, there is a need for a
more rened approach in those cases where the original soures maintain
their own independent view of the world.

In distributed environments, ontology engineers want to reuse third party ontologies or, even more, parts of existing
ontologies, while maintaining consistency, at least in their local knowledge representation.

However, it has been often
noted, that although DLs are well-suited for representing a single, global viewpoint on an application domain,
they offer no formal grounding for dealing with knowledge pertaining to multiple heterogeneous viewpoints
— a scenario ever more often approached in practical
applications, e.g. concerned with reasoning over distributed knowledge sources on the Semantic Web.

Under the standard
Kripkean semantics, a DL ontology forces a unique, global
view on the represented world, in which the ontology axioms are interpreted as universally true. This philosophy is
well-suited as long as everyone can share the same conceptual perspective on the domain or there is no need for considering alternative viewpoints. Alas, this is hardly ever the
case and very often, same domains are modeled differently
depending on the intended use of an ontology. In practice,
effective representation and reasoning about knowledge pertaining to such multiple heterogenous viewpoints becomes
the primary objective for many applications, e.g. those concerned with reasoning over distributed knowledge sources on the Semantic Web (Guha, McCool, and Fikes 2004;
Bao et al. 2010).
The challenges above resemble clearly the problems
which once inspired J. McCarthy to introduce his theory of
formalizing contexts in knowledge representation systems,
as a way of granting them more generality (McCarthy 1987;
Guha 1991). The gist of his proposal, motivating several
existing logics of context (Buvac and Mason 1993; Buva ˇ cˇ
1996; Nossum 2003), is to replace logical formulas ϕ, as the
basic knowledge carriers, with assertions ist(c, ϕ). Assertions of this form state that ϕ is true in c, where c denotes an
abstract first-order entity called a context, which on its own
can be described in a first-order language.

The formalism proposed in this paper incorporates these
fundamental ideas of McCarthy’s theory into the DL framework by considering contexts as abstract, first-class citizens,
and offering an expressive formal apparatus for modeling
their semantic interoperability. As a result, we harmonize
and give a uniform formal treatment to two seemingly diverse aspects of the problem of reasoning with contexts in
DL: 1) how to extend DLs to support the representation of
inherently contextualised knowledge; 2) how to use knowledge from coexisting classical DL ontologies while respecting its context-specific scope. Our logic is essentially a twodimensional DL, in the style of product-like combinations
of DLs with modal logics (Wolter and Zakharyaschev 1999;
Kurucz et al. 2003), similar to e.g. temporal DLs (Lutz,
Wolter, and Zakharyaschev 2008; Artale, Lutz, and Toman
2007). In particular, we extend the standard DL semantics
with a second dimension, representing a possibly infinite
domain of contexts, and include additional modal operators
along with a separate metalanguage in the syntax, for quantifying and expressing properties over the context entities.



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%Natural language terms do not have precise, universally agreed definitions that fix their meanings  \cite{Wittgenstein1958PhilosophicalInvestigations}. Instead, their applicability is unclear in some instances, and it may vary depending on the context and pragmatics of use. Thus, when an agent formalises a domain, the resulting conceptual model will be shaped by her own world-view and by pragmatic factors, such as the context, intended granularity and scope. %Unavoidably, different agents and contexts of application bring up different conceptualisations. 

The notion \emph{safe}, for instance, is a paradigmatic case of this effect. Its semantics can be described as a \emph{family resemblance}, shifting from ``not being in danger'', to ``not being dangerous'', passing by ``cautious'' and ``dependable'' among other. Even when we restrict ourselves to a specific and applied domain, such as the safety of medical devices, different agents and institutions may hold different standpoints. Consder the following (fictional) example:

\begin{example}\label{example:medical-devices}
    According to EU regulation, a device that has a risk is not safe, and needs to go through a process to justify the mitigation of such risk. State members comply with this regulation and further specify it. According to German regulation, a device with an exposed needle is a risky device. French regulation considers that needles with protection caps are safe parts of devices.
\end{example}

While ontologies and knowledge bases are aimed at providing a common vocabulary for representing shared knowledge \cite{Guarino1998}, the described semantic heterogeneity may hinder the interoperation of independently developed systems. Ontology integration is well-studied yet still challenging \cite{Kalfoglou2003OntologyArt,Euzenat2008OntologyAlignments,Otero-Cerdeira2015OntologyReview}, and merging knowledge sources often involves a certain knowledge loss or weakening in order to avoid incoherence and inconsistency \cite{Pesquita2013ToAlignments,Solimando2017MinimizingEvaluation}.
In contrast, we advocate a multi-perspective approach that can represent and reason with many -- possibly conflicting -- standpoints, instead of focusing on combining and merging different sources into a single conflict-free conceptual model.

\emph{Standpoint logic} \cite{gomez2021standpoint} is a simple formalism rooted in modal logic that supports the coexistence of multiple \emph{standpoints} and the establishment of alignments between them. In the original work \cite{gomez2021standpoint}, the framework is introduced with a propositional base. While good complexity results are shown (it stays in \textsc{NP} like its  base language), it is arguable that the framework is not expressive enough for most knowledge integration scenarios.

In this paper we present a first-order extension of standpoint logic. We provide the syntax and semantics and extend the language to support set-theoretical combinations of standpoints (Section \ref{sec:fol-standpoint-logic}). Then, we show how a small model property can be shown for the \emph{sentential} fragment, which imposes restrictions on the use of standpoint operators (Section \ref{sec:small-model-property}). Tailored to this case, we introduce a fragment-preserving translation (Section \ref{sec:translation}) that is polynomial on the size of the formula, with which not only we can establish complexity bounds for some subfragments but also directly use of-the-shelf reasoners. We demonstrate this by extending our results to a standpoint logic based on the description logic $\SROIQbs$, a semantic fragment of FOL closely related to the OWL~2~DL ontology language, and we illustrate some typical use cases with an example in the medical domain (Section \ref{sec:example-medical}).

==> sections/Medical-example.tex <==
Let us consider an example in the domain of medical devices.

Below is a tentative list of desirable elements of an example.
\begin{itemize}
	\item Two standpoints that are disjoint, so we can infer this property.
	\item Two standpoints that subsume eachother.
	\item The union of two standpoints. By knowing that one element does not fit one, we can infer that it fits the other.
	\item Inference of necessary (box), possible (diamond) and indefinite facts (I).
\end{itemize}

For instance, consider the following example:
\begin{gather}
	\mathsf{FR} \preceq \mathsf{EU} \sqcap \mathsf{DE} \preceq \mathsf{EU}\\%\standbx{EU} \pred{Device} \sqcap \exists\pred{hasRisk}\sqsubseteq \pred{RiskDevice}\\
	\standbx{EU} \pred{RiskDevice} \sqcap \pred{SafeDevice} \equiv \bot\\
	\pred{Device} \sqsubseteq \pred{RiskDevice} \sqcup \pred{SafeDevice} \\
	\standbx{DE}\pred{RiskDevice} \sqsubseteq \role{hasExposedPart}.\pred{Needle}\\
	\standbx{FR}\pred{SafeDevice} \sqsubseteq \n \exists\role{hasPart}.\pred{RiskyPart}\\
	\standbx{FR}\pred{NeedleWithProtectionCap}\sqsubseteq\pred{SafePart}\\
	\allstandb \pred{NeedleWithProtectionCap} \sqsubseteq \pred{Needle}\\
	\pred{Device}(\#005)\\
	\pred{NeedleWithProtectionCap}(\#003)\\
	\pred{hasExposedPart}(\#005,\#003)
\end{gather}

From this example we can infer knowledge about the standpoints themselves, namely that $\mathsf{FR} \npreceq \mathsf{DE}$ and $\mathsf{DE} \npreceq \mathsf{FR}$, that is, that they are \emph{incompatible}.
In addition, we can infer facts relative to the different standpoints, such as that while the french regulation considers $\#005$ safe, the German one does not, and thus according to the EU it is inherently indeterminate.
\begin{gather}
	\n(\mathsf{FR} \preceq \mathsf{DE}) \sqcap \n(\mathsf{DE} \preceq \mathsf{FR})\\
	\standbx{FR}\pred{SafeDevice}(\#005)\\
	\standbx{DE}\neg\pred{SafeDevice}(\#005)\\
	\standindef{EU}\pred{SafeDevice}(\#005)
\end{gather}

Note that indeterminacy is different from our inference that $\standdx{EU}\exists\role{hasExposedPart}.\pred{Needle}\sqsubseteq\pred{RiskDevice}$, which states that any device with an exposed needle is considered risky in at least some interpretations (and potentially in some of them).

Finally, let us say that for a product to be viable for production, it must be considered safe in at least one of the target countries, in this case only Germany ({\sf DE}) and France ({\sf FR}). Let us now build on the previous example with the following assertions,

\begin{gather}
	\standbx{FR}\exists\role{hasExposedPart}.\pred{Hot}\sqsubseteq\pred{RiskDevice}\\
	\pred{Hot}(\#006)\\
	\exists\pred{hasExposedPart}(\#005,\#006)
\end{gather}

From this, we can infer that $\negstanddx{FR\cup DE}\pred{SafeDevice}(\#005)$, in other words, across all interpretations and for different reasons it is the case that $\standbx{FR\cup DE}\pred{RiskDevice}(\#005)$.


==> sections/Medical-example3.tex <==
\section{FOL Example in a Medical Ontology}
Let us consider an example in the domain of medical devices.

% Below is a tentative list of desirable elements of an example.
% \begin{itemize}
% 	\item Two standpoints that are disjoint, so we can infer this property.
% 	\item Two standpoints that subsume eachother.
% 	\item The union of two standpoints. By knowing that one element does not fit one, we can infer that it fits the other.
% 	\item Inference of necessary (box), possible (diamond) and indefinite facts (I).
% \end{itemize}

\begin{gather}
	\mathsf{FR} \preceq \mathsf{EU} \con \mathsf{DE} \preceq \mathsf{EU}\\%\standbx{EU} \pred{Device} \sqcap \exists\pred{hasRisk}\sqsubseteq \pred{RiskDevice}\\
	\standbx{EU} \forall x \pred{MedDevice}(x) \dimp (\pred{AI}(x) \dis \pred{IVD}(x) \dis \pred{OMD}(x))\\
	%\mathsf{FR} \preceq \mathsf{EU} \sqcap \mathsf{DE} \preceq \mathsf{EU}\\
	%\standbx{EU} \pred{RiskDevice} \sqcap \pred{SafeDevice} \equiv \bot\\
	\pred{Device} \sqsubseteq \pred{RiskDevice} \sqcup \pred{SafeDevice} \\
	\standbx{DE}\pred{RiskDevice} \sqsubseteq \role{hasExposedPart}.\pred{Needle}\\
	\standbx{FR}\pred{SafeDevice} \sqsubseteq \n \exists\role{hasPart}.\pred{RiskyPart}\\
	\standbx{FR}\pred{NeedleWithProtectionCap}\sqsubseteq\pred{SafePart}\\
	\allstandb \pred{NeedleWithProtectionCap} \sqsubseteq \pred{Needle}\\
	\pred{Device}(\#005)\\
	\pred{NeedleWithProtectionCap}(\#003)\\
	\pred{hasExposedPart}(\#005,\#003)
\end{gather}

From this example we can infer knowledge about the standpoints themselves, namely that $\mathsf{FR} \npreceq \mathsf{DE}$ and $\mathsf{DE} \npreceq \mathsf{FR}$, that is, that they are \emph{incompatible}.
In addition, we can infer facts relative to the different standpoints, such as that while the french regulation considers $\#005$ safe, the German one does not, and thus according to the EU it is inherently indeterminate.
\begin{gather}
	\n(\mathsf{FR} \preceq \mathsf{DE}) \sqcap \n(\mathsf{DE} \preceq \mathsf{FR})\\
	\standbx{FR}\pred{SafeDevice}(\#005)\\
	\standbx{DE}\neg\pred{SafeDevice}(\#005)\\
	\standindef{EU}\pred{SafeDevice}(\#005)
\end{gather}

Note that indeterminacy is different from our inference that $\standdx{EU}\exists\role{hasExposedPart}.\pred{Needle}\sqsubseteq\pred{RiskDevice}$, which states that any device with an exposed needle is considered risky in at least some interpretations (and potentially in some of them).

Finally, let us say that for a product to be viable for production, it must be considered safe in at least one of the target countries, in this case only Germany ({\sf DE}) and France ({\sf FR}). Let us now build on the previous example with the following assertions,

\begin{gather}
	\standbx{FR}\exists\role{hasExposedPart}.\pred{Hot}\sqsubseteq\pred{RiskDevice}\\
	\pred{Hot}(\#006)\\
	\exists\pred{hasExposedPart}(\#005,\#006)
\end{gather}

From this, we can infer that $\negstanddx{FR\cup DE}\pred{SafeDevice}(\#005)$, in other words, across all interpretations and for different reasons it is the case that $\standbx{FR\cup DE}\pred{RiskDevice}(\#005)$.


==> sections/Motivation.tex <==

\emph{Standpoint Logic} \cite{gomez2021standpoint} is a lightweight multi-modal framework where labelled modalities $\standbs$ express information relative to a standpoint, and the set of formulas preceded by a standpoint operator (i.e., expressions of the form $\standbs\phi$ or $\standds\phi$) represent the agent's world-view or semantic commitments.\footnote{For clarity and better readability, we will sometimes use square brackets $[\,\cdots]$ to explicitly indicate the scope of modal operators.}

Standpoint logic draws from the philosophical theory of supervaluationism, according to which the phenomenon of vagueness (and more generally semantic variability) can be explained by the fact that natural language can be interpreted in many different yet equally acceptable ways \cite{Keefe1997TheoriesVagueness}, commonly referred to as \emph{precisifications}. 
When using a modal infrastructure in a supervaluationistic framework, the usual structure of \emph{possible worlds} is replaced by one of \emph{precisifications}. Thus, in contrast to doxastic frameworks, settings like the one in \Cref{example:medical-devices} do not require standpoint operators to be nested, and there is no \emph{actual world} that could dictate what is contingently true, as the German and the French worldviews are both to be valued equally.

%To see the difference, consider a situation modelled with doxastic logic: Bob believes that there is a red apple at home ($B_{Bob}[\pred{red\_apple}]$) and Tim believes that there is a yellow apple instead, ($B_{Tim}[\pred{yellow\_apple}]$). Here, the possible worlds model the different possible states of affairs, and there is an  \emph{actual world} that dictates what is contingently true. In contrast, consider Tim and Bob facing a  red/yellowish apple. Tim calls it a red apple ($\standb{Tim}[\pred{red\_apple}]$), yet Bob calls it a yellow apple, ($\standb{Bob}[\pred{yellow\_apple}]$). The latter is what standpoint logic models, where agents describe the state of the matter using different and equally acceptable interpretations of the vocabulary, so there is no \textquote{actual precisification}. 

%Different modal frameworks have been proposed in the supervaluationist literature \cite{Varzi2007SupervaluationismLogics,Williams2008SupervaluationismRevisionism,Cobreros2011SupervaluationismLogic}. These focus on proposing modalities that can capture the linguistic behaviour of philosophical vagueness and the sorites paradox, and on the analysis of different forms of validity and logical consequence. In contrast, we focus on scenarios where different agents or different contexts are linked to different usages of such a semantically variable language.  

%Standpoints are modelled as non-empty sets of \emph{precisifications}, which corresponds to the intuition that a standpoint is (typically) a \emph{partial} semantic commitment that can be made fully precise in different ways. 
In terms of syntax, the standpoint framework exhibits a reasonable versatility through a very economic extension of the FOL base language by constants~$\spform{s}$ and combinations thereof for denoting standpoints -- with the special constant~\star denoting the global standpoint -- and corresponding pairs of dual modal operators $\standbs$ and $\standds$. 

\begin{enumerate}[label={\bf \arabic*.},ref={\bf \arabic*}] 
	\item[$\standbs\phi$] (or $\allstandb\phi$) reads as ``It is unequivocal, [from the point of view \emph{s},] that $\phi$". This is the paradigmatic form of a semantic commitment (in the case of \star, the statement is global, i.e., universally agreed upon).
	
	\item[$\standds\phi$] (or $\allstandd\phi$) reads as ``[From the point of view \emph{s},] in some sense $\phi$''. In practice, this means that the standpoint \st (or \star) has no argument to rule out $\phi$, and hence, it is acceptable to interpret \st (or \star) in such a way that $\phi$ holds.
\end{enumerate} 


Practical uses of \emph{standpoint logic} include, for instance, the representation of multiple (and possibly conflicting) symbolic conceptualisations of a domain, knowing what can be inferred from the consensual semantics of sets of agents and knowing which standpoints are compliant with a partial truth. 
For instance, in \Cref{example:medical-devices}, we can represent and infer (a) global or standpoint-relative statements,  (b) unequivocal,  and \textquote{\emph{in some sense}} statements, (c) hierarchies and globality of standpoints, such as $(\spform{EU}\preceq\spform{FR})$, which models that the standpoint $\spform{FR}$ is \textquote{subsumed} by the standpoint $\spform{EU}$, and (d) \textquote{complex alignments} between standpoints, such as 
%$\forall x \underset{FR}{\square}\pred{SafeDev}(x)\imp(\underset{DE}{\lozenge}\pred{SafeDev}(x)\con  \underset{DE}{\square}\n\pred{Forbidden}(x))$
$\forall x {\square}_\spform{FR}\pred{SafeDev}(x)\imp({\lozenge}_\spform{DE}\pred{SafeDev}(x)\con  {\square}_\spform{DE}\n\pred{Forbidden}(x))$
Intuitively, the latter would mean that, whenever a device X is unequivocally safe according to $\spform{FR}$, we know that it is at least in some sense safe according to $\spform{DE}$ and definitely not forbidden.


%In the rest of this section, we demonstrate how to specify Example~\ref{example:first-colours} using simple statements of the kinds (a) and (b), and we will present some of the inferences that we can obtain. Later, in Section \ref{sec:last-examples-applications}, we will address more complex statements of the kinds (c) and (d) by extending and enriching the same example, after presenting the formal specification of the language in Section \ref{sec:formal-language}. 

%From this, we can derive the expected facts for each theory/standpoint specifically, such as \textquote{Unequivocally, according to $CT$, if a colour is lime then it is not yellow} ($\standb{CT} [\pred{Lime}\imp\n\pred{Yellow}]$), and general findings, such as \textquote{Under some interpretations, colours can be classified into cold and warm} ($\allstandd[\pred{Colour}\imp(\pred{CC}\dis\pred{WC})]$).

The crucial aspect of this framework in contrast to the merging strategy discussed in \Cref{sec:introduction} is that the former sentences are not inconsistent, so all axioms and known alignments can be jointly represented. Standpoint logic escapes global inconsistency, without removing alignments or relations and avoiding the duplication of entities, because the model theory based on Kripke-structures (cf.~\Cref{sec:fol-standpoint-logic}) forces consistency only within standpoints and precisifications, but allows for the specification of sets of standpoints that are mutually inconsistent, which are modelled as disjoint sets.

%%%% CHECK THESE COMMENTS FOR THE FINAL WRITE UP

%\extra{We typically establish standpoints by setting constraints (axioms and threshold limitations such as \ref{EG:deftall} and \ref{EG:ttall}) and through implicit commitments (asserting that a predicate holds or does not hold for an object of the domain such as \ref{EG:shortnena}) that pick out a corresponding set of admissible precisifications that satisfy them. }

%   \extra{Since they are modelled as sets, standpoints form a lattice under the subset relation; and, when one standpoint is a subset of another, we may also regard it as more precise, since it rules out certain interpretations of the vocabulary (this is expressed by \ref{EG:subs}).}

%  \extra{Overall, standpoints provide a simple formal mechanism that not only preserves the supervaluationist treatment of vagueness as proposed in the philosophical literature, but it also extends the expressive capacities of the framework to the needs of multi-agent systems, further capturing  philosophical intuitions that highlight the inherent ties between the semantics of terms and the use to which language is put. In turn, this expands the versatility of the framework, as we will explore in Section \ref{sec:representation}, while formally maintaining a simple logic that is relatable to the well established epistemic multi-modal logics but that has better computational properties because of its stronger axiomatisation.}



\iffalse

\section{Standpoint Framework}

In standpoint logic, a \emph{precisification\/} is identified with a precise interpretation of the language, such that every word has a unique, sharp definition. The definitional theory may involve additional axioms and it must be consistent, such that for any state of the world there is a unique extension for every predicate.

\alert{TODO: This notion is borrowed from the supervaluationist theory of vagueness, for which modal frameworks have been given. Add a short paragraph long introduction.}

Once we have a framework that models the semantic variability of language in terms of a set of \emph{precisifications} or precise languages, the notion of \emph{standpoint} responds to the intuition that when an agent makes use of such language, she is unlikely to use a particular \emph{precisification}. For instance, she is unlikely to commit to a fully precise language before referring to someone as \emph{tall}. \lg{Instead, agents typically limit themselves to make the minimal commitments on the terms and relations that are relevant for them in order to communicate effectively (modularity). \reword{A standpoint is the set of languages that are compatible with these comitments:}
	%Our framework interprets the semantics of the vague language as a collection of admissible precisifications of the language. 
	\lg{they capture the intuition that an agent commits to the subset of precise interpretations of the language that are consistent with her own statements\footnote{This is presumed on the basis of general communication principles, for example supported by \cite{Grice1975LogicConversation}. The contrary would be regarded as a dishonest behaviour from the agent, which we do not model in this framework.}.}}\lgcomment{remove?}. 


\fi

==> sections/Notes-fragments.tex <==

\subsection{Possible Fragments}

\subsubsection{Straightforward Fragments}
\begin{itemize}
	\item Rigid identifiers (rigid constant and function symbols): $\gamma(\pr)$ must agree on $\Funcs$ over all $\pr\in\Precs$ in every $\kstruct$.
	\item Modalities only in front of sentences: formulas of the form $\standbs\phi$ are only allowed when $\phi$ does not contain free occurrences of variables.
\end{itemize}

\subsubsection{Standpoint \EL}
We allow no function symbols of arity greater than zero, and no predicate symbols of arity greater than two;
we allow only two variables $x, y$.
We denote unary predicates by $C, C_1, C_2, \ldots$,
binary predicates by $R, R_1, R_2, \ldots$,
constants by $a, a_0, a_1, \ldots$,
standpoint symbols by $s, s_1, s_2$.

We allow only the following forms of formulas\/:\todo{Find out if we can allow standpoint boxes in standpoint \EL.}
\begin{align*}
	\intertext{Concept formulas (dually defined for the free variable $y$):}
	\phi(x) & \ebnfeq C(x) \mid \phi_1(x) \land \phi_2(x) \mid \exists y(R(x,y) \land \phi(y)) \mid \standds\phi(x) \ebnfoptional{\standbs\phi(x)}
	\intertext{general concept inclusions:}
	\psi    & \ebnfeq \forall x (\phi_1(x) \limplies \phi_2(x)) \mid \standds\psi \ebnfoptional{\standbs\psi}
	\intertext{assertions:}
	\xi     & \ebnfeq P(a) \mid R(a_1,a_2) \mid s_1\cap s_2\preceq s \mid \neg\xi \mid \standds\xi
\end{align*}
A standpoint~\EL knowledge base $T$ is then a set of general concept inclusions and assertions;
an interpretation $\kstruct$ is a \define{model} for $T$ if and only if it is a model for all formulas $\psi,\xi\in T$.

Our hope is that the restriction to \EL will recover the small model property.
\begin{conjecture}
	Let $T$ be a standpoint \EL knowledge base and $\kstruct=\tuple{\Dom,\Precs,\sigma,\gamma}$ be a model for $T$.

	There exists a model $\kstruct'$ whose size is at most polynomial in the size of $T$.
	\begin{proof}
		We consider the set $\Sub(T)=\bigcup_{\zeta\in T}\Sub(\zeta)$ and define the set of canonical precisifications:
		\begin{multline*}
			\Precs_T = \set{ \pr_\xi \guard \standds\xi\in\Sub(T) } \cup \set{\pr_{\neg s_1\cap s_2\preceq s} \guard \neg s_1\cap s_2\preceq s\in\Sub(T) } \cup \\
			\set{ \pr_\psi \guard \standds\psi\in T } \cup \set{ \pr_\phi \guard \standds\phi\in\Sub(T) }
		\end{multline*}
		Basically, we could define $\Precs_T=\set{\pr_\zeta \guard \standds\zeta\in\Sub(T) }$, but we might want to be able to distinguish whether a precisification is due to a concept formula or due to an axiom.
		We now continue defining $\kstruct'=\tuple{\Dom,\Precs_T,\sigma',\gamma'}$ along with a relation ${\sim} \subseteq \Precs\times\Precs_T$ as follows.
		(The intution behind $\sim$ is that $\pr\sim\pr_\zeta$ iff the witnessing capabilities of $\pr$ should be transferred to $\pr_\zeta$ during the construction.)

		We know that $\kstruct$ is a model for $T$, so for each general concept inclusion $\psi\in T$, we have $\kstruct,\pr\models\psi$ for all $\pr\in\Precs$.
		We do a case distinction on the syntactic form of $\psi$:
		\begin{description}
			\item[\normalfont$\psi=\forall x(\phi_1(x)\limplies\phi_2(x))$:]
			      Then for each $\pr\in\Precs$ and domain element $\de\in\Dom$, we have that $\kstruct,\pr,\set{x\mapsto\de}\models\phi_1(x)\limplies\phi_2(x)$.
			      In other words,
			      (1) $\kstruct,\pr,\set{x\mapsto\de}\not\models\phi_1(x)$, or
			      (2) $\kstruct,\pr,\set{x\mapsto\de}\models\phi_2(x)$.
			      \begin{enumerate}
				      \item $\kstruct,\pr,\set{x\mapsto\de}\not\models\phi_1(x)$:
				            We do a case distinction on the syntactic form of $\phi_1(x)$.
				            \begin{description}
					            \item[\normalfont$\phi_1(x)=C(x)$:]
					                  Then $\kstruct,\pr,\set{x\mapsto\de}\not\models C(x)$, that is, $\de\notin\interpret{C}{\gamma(\pr)}$.
					            \item[\normalfont$\phi_1(x)=\phi_3(x)\land\phi_4(x)$:]
					                  We continue recursively with whichever of $\kstruct,\pr,\varassign\not\models\phi_3(x)$ or $\kstruct,\pr,\varassign\not\models\phi_4(x)$ is true (at least one of them is).
					            \item[\normalfont$\phi_1(x)=\exists y(R(x,y)\land\phi_3(y))$:]
					                  Then for each $\de'\in\Dom$ we find $\kstruct,\pr,\set{x\mapsto\de,y\mapsto\de'}\not\models R(x,y) \land \phi_3(y)$.
					                  Thus for all $\de'\in\Dom$ such that $\tuple{\de,\de'}\in\interpret{R}{\gamma(\pr)}$, we continue recursively with $\kstruct,\pr,\set{x\mapsto\de,y\mapsto\de'}\not\models\phi_3(x)$.
					                  \todo{This should be fine as long as we do not introduce as many pairs into $\sim$ as there are $\de'\in\Dom$ below this point.}
					            \item[\normalfont$\phi_1(x)=\standds\phi_3(x)$:]
					                  Then for each $\pr'\in\sigma(s)$ we continue recursively with $\kstruct,\pr',\set{x\mapsto\de}\not\models\phi_3(x)$.\todo{This should be fine as long as we are not forced to put every $\pr'\in\sigma(s)$ into $\sim$ for some subformula of $\phi_3(x)$.}
				            \end{description}
				      \item $\kstruct,\pr,\set{x\mapsto\de}\models\phi_2(x)$:
				            We do a case distinction on the syntactic form of $\phi_2(x)$.
				            \begin{description}
					            \item[\normalfont$\phi_2(x)=C(x)$:]
					                  Then $\kstruct,\pr,\set{x\mapsto\de}\models C(x)$, that is, $\de\in\interpret{C}{\gamma(\pr)}$.
					            \item[\normalfont$\phi_2(x)=\phi_3(x)\land\phi_4(x)$:]
					                  We continue recursively with $\kstruct,\pr,\varassign\models\phi_3(x)$ and $\kstruct,\pr,\varassign\models\phi_4(x)$.
					            \item[\normalfont$\phi_2(x)=\exists y(R(x,y)\land\phi_3(y))$:]
					                  Then there is a $\de'\in\Dom$ such that $\kstruct,\pr,\set{x\mapsto\de,y\mapsto\de'}\models R(x,y) \land \phi_3(y)$.
					                  That is, $(\de,\de')\in\interpret{R}{\gamma(\pr)}$ and $\kstruct,\pr,\set{x\mapsto\de,y\mapsto\de'}\models\phi_3(y)$, continuing recursively.
					            \item[\normalfont$\phi_2(x)=\standds\phi_3(x)$:]
					                  Then there is a $\pr'\in\sigma(s)$ such that $\kstruct,\pr',\set{x\mapsto\de}\models\phi_3(x)$.
					                  We set $\pr'\sim\pr_{\phi_3}$ and continue recursively.
				            \end{description}
			      \end{enumerate}
			\item[\normalfont$\psi=\standds\psi_1$:]
			      Then there is a $\pr\in\sigma(s)$ such that $\kstruct,\pr\models\psi_1$.
			      We set $\pr\sim\pr_{\psi_1}$ for this specific $\pr$.
			      Furthermore, using the premise $\kstruct,\pr\models\psi_1$ we continue the construction recursively.
		\end{description}
		Likewise, we know that $\kstruct$ is a model for each assertion $\xi\in T$, that is, $\kstruct,\pr\models\xi$ for all $\pr\in\Precs$.
		We do a case distinction on the syntactic form of $\xi$:
		\begin{description}
			\item[\normalfont$\xi=P(a)$:]
			      Then $\interpret{a}{\gamma(\pr)}\in\interpret{P}{\gamma(\pr)}$.
			\item[\normalfont$\xi=R(a_1,a_2)$:]
			      Then $\tuple{\interpret{a_1}{\gamma(\pr)},\interpret{a_2}{\gamma(\pr)}}\in\interpret{R}{\gamma(\pr)}$.
			\item[\normalfont$\xi=s_1\cap s_2\preceq s$:]
			      Then $\sigma(s_1)\cap\sigma(s_2)\subseteq\sigma(s)$.
			\item[\normalfont$\xi=\neg\xi_1$:]
			      Then $\kstruct,\pr,\varassign\not\models\xi_1$.
			      We do a case distinction on the syntactic form of $\xi_1$:
			      \begin{description}
				      \item[\normalfont$\xi_1=P(a)$:]
				            Then $\interpret{\gamma(\pr)}{a}\notin\interpret{P}{\gamma(\pr)}$.
				      \item[\normalfont$\xi_1=R(a_1,a_2)$:]
				            Then $\tuple{\interpret{a_1}{\gamma(\pr)},\interpret{a_2}{\gamma(\pr)}}\notin\interpret{R}{\gamma(\pr)}$.
				      \item[\normalfont$\xi_1=s_1\cap s_2\preceq s$:]
				            Then there is some $\pr'\in\sigma(s_1)\cap\sigma(s_2)\setminus\sigma(s)$.
				            We record $\pr'\sim\pr_{\neg s_1\cap s_2\preceq s}$.
				      \item[\normalfont$\xi_1=\neg\xi_2$:]
				            We continue recursively with $\kstruct,\pr,\varassign\models\xi_2$.
				      \item[\normalfont$\xi_1=\standds\xi_2$:]
				            Then for all $\pr'\in\sigma(s)$, we find that $\kstruct,\pr',\varassign\not\models\xi_2$ and treat all such cases recursively.
			      \end{description}
			\item[\normalfont$\xi=\standds\xi_1$:]
			      Then there is some $\pr'\in\sigma(s)$ such that $\kstruct,\pr',\varassign\models\xi_1$.
			      We record $\pr'\sim\pr_{\xi_1}$ and continue recursively.
		\end{description}
		We note that for every subformula $\zeta\in\Sub(T)$ of the form that is relevant to $\Precs_T$, we will have collected at least one $\pr\in\Precs$ such that $\pr\sim\pr_{\zeta}$.

		Assuming that we have defined $\sim$ in this way, we proceed to define\/:
		\begin{align*}
			\sigma' & :\Stands\to 2^{\Precs_T}, & s         & \mapsto \set{ \pr_\zeta\in\Precs_T \guard \exists\pr'\in\sigma(s) \pr'\sim\pr_\zeta } \\
			\gamma' & :\Precs_T\to \Structs,    & \pr_\zeta & \mapsto \gamma(\pr) \text{ for some } \pr\in\Precs \text{ with } \pr\sim\pr_\zeta
		\end{align*}
		Essentially, the “worlds” $\gamma(\pr)$ do not change, we only re-assign some of the worlds $\gamma(\pr)$ to new precisification symbols $\pr_\zeta$.
		Those new precisification symbols are in turn assigned to standpoint constants as dictated by $\sim$.
		It is easy to see that there are at most as many precisifications $\pr_\zeta\in\Precs_T$ as there are $\standds$ (and $\neg s_1\cap s_2\preceq s$) subformulas in $T$.
		Whenever for each $\pr_\zeta$ there is a $\pr\in\Precs$ with $\pr\sim\pr_\zeta$, the function $\gamma'$ above is well-defined.

		It remains to show that $\kstruct'$ is indeed a model for $T$.
		\todo{Continue here.}
	\end{proof}
\end{conjecture}

\subsubsection{Standpoint \FL}
Like standpoint~\EL, but with $\forall y(R(x,y)\limplies \phi(y))$ in place of existential restriction, and $\standbs$ instead of $\standds$ in concept formulas.

\subsection{Some notes by Sebastian}

Some results for Standpoint-DLs with modalities prededing open subformulas.

\subsubsection{Modalities for Roles are Dangerous}

Take $\mathcal{ALCHOIF}$ TBoxes, just the universal standpoint $\ast$ and allow modalities $\Box_\ast$ and $\Diamond_\ast$ in front of axioms and role names. Then satisfiability is undecidable.
Proof Idea: axiomatize an infinite grid of $H$ and $V$ roles, on which a tiling problem can be expressed.

\subsubsection{Modalities for Concepts are OK}

Take $\mathcal{SHIQ}b$ KBs. We allow for sharpening statements of the form $s_1 \cap s_2 \preceq s_3$, but only standpoint symbols in boxes and diamonds, which are allowed to occur in front of whole axioms or of concept expressions. In particular, no Boolean operators connecting DL axioms are allowed.
Then, the polynomial model property is satisfied. This allows for a polynomial satisfiability-preserving translation into $\mathcal{SHIQ}b$, leading to \textsc{ExpTime}-complete satisfiability checking.

Proof Idea: The class of models of a $\mathcal{SHIQ}b$ KB is closed under disjoint union. If we heavily use this property together with the insight that for normalised KBs, we can ``re-wire'' identity of domain elements if we obey 1-types, we can squeeze many ``witness worlds'' into one, getting the number of worlds down to polynomially many.

\bigskip

Take theories of two-variable FOL with counting quantifiers (denoted $\mathcal{C}^2$). We allow for full standpoint algebra. Boxes and Diamonds are allowed to occur in front of sentences and formulae with 1 free variable. Satisfiability in such a logic is \textsc{NExpTime}-complete, just as for plain $\mathcal{C}^2$.

Proof idea: First establish that for every satisfiable such theory, a collection of exponentially many ``witness worlds'' is sufficient to verify satisfiability. Second show how these worlds can be combined into one plain $\mathcal{C}^2$-model which can be characterised by a $\mathcal{C}^2$-theory that has a polynomially larger signature than the original one. Notably the length of the theory may be exponential in the original one but that doesn't harm us.

This result can be leveraged to show that for $\mathcal{SHOIQ}$ and $\mathcal{SROIQ}$ KBs (i.e., OWL 1 and OWL 2 DL), standpoints can be added to the logic while still remaining in the same complexity class. However, a reduction to reasoning in the base logics (as it was done above for $\mathcal{SHIQ}b$) remains elusive.


==> sections/Other-examples.tex <==
\section{Other Examples}
On the motivation example at the beginning of this paper we explore a scenario where the preservation of the standpoints of FR and GE is necessary. 
Let us consider now usual knowledge integration scenarios extracted from an experiment in \cite{Osman2021OntologyIssues}, on the holistic integration of three ontologies (using pairwise alignments) from the \emph{LargeBio} track of the Ontology Alignment Evaluation Initiative 2020 \cite{NikooiePour2020Results2020}. These are: the FMA (Foundational Model of Anatomy), the SNOMED-CT (Clinical Terms), and the NCI (National Cancer Institute Thesaurus). In what follows, we will refer to the entities of these sources by their initials, for the sake of compactness.

\Cref{fig:example_lymph_node} illustrates a snippet from the alignments found between FMA and SNOMED-CT in the left and an integration in the right. The integration displays subsumption redundancies and a subsumption cycle formed because of the addition of two equivalence correspondences having the same source class \textquote{001\#Abdominal\_lymph\_node} (ALN), resulting in three equivalent classes merged together to constitute a single class. The proposed alternative in \cite{Osman2021OntologyIssues} is to give up on one of the two alignments, hence concluding either $ANL\equiv ANLG$ or $ANL\equiv ANLS$, but not both. 

\begin{figure}[b]
	\includegraphics[width=26em]{images/01.jpg}
	\caption{Example 1}\label{fig:example_lymph_node}
\end{figure}   

Let us consider that the output of the merge process is represented under a standpoint that we name $\mathsf{A12}$, and it contains assertions relevant to all the statements that are not flagged as problematic. Then, we state:

\begin{enumerate}[series=osmanExamples,label={(E7-\arabic*).},ref={\bf E7-\arabic*},leftmargin=3.4em,labelwidth=4em] 
        \item $\mathsf{A12} \preceq \mathsf{(A1\cup A2)}$\label{formula:osmanEx1L1}
        \item $\standb{A1}[\pred{ALN}\dimp\pred{ALNS}]\ \con \ \standb{A2}[\pred{ALN}\dimp\pred{ALNG}]$\label{formula:osmanEx1L3}
\end{enumerate}

Line \ref{formula:osmanEx1L1} states that any acceptable interpretation of our standpoint $\s{(\#001+2)}$ must be acceptable for $\standb{A1}$ or for $\standb{A2}$ (or both), hence forcing to take at least one disambiguation. Then, the line \ref{formula:osmanEx1L3} formalises the alternative equivalences. 

This contrasts with the previous examples, where a more modular approach was taken and referring to the most specific standpoints was interesting. Here, in the context of large ontologies, that level of detail would be unrealistic, and we are likely to only be interested in more general inferences such as:

 \begin{enumerate}[label={(\arabic*).},ref={\bf \arabic*},leftmargin=1.8em,labelwidth=2em] 
        \item $\standb{(\#001+2)}[(\pred{ALN}\imp\pred{ALNS})\ \con \ (\pred{ALNG}\imp\pred{ALN})]$\label{formula:osmanEx1L5}
        \item $\standd{(\#001+2)}[\pred{ALN}\dimp\pred{ALNS}]\con\standd{(\#001+2)}[\pred{ALN}\dimp\pred{ALNG}]$\label{formula:osmanEx1L7}
\end{enumerate}

This means that we will not have conflicts if we know of (a) one instance of $\pred{ALN}$ not being $\pred{ALNG}$ or (b) one instance of $\pred{ALNS}$ not being $\pred{ALN}$, which would clash with the alignment approach. 


\begin{figure}[b]\label{fig:example_2}
	\includegraphics[width=26em]{images/03.jpeg}
	\caption{Example 3}
\end{figure}   

==> sections/Propositional-standpoint-logic.tex <==

We attempt to translate propositional standpoint logic to classical propositional logic in a way that allows a straightforward generalisation to first-order logic that does not increase the arity of involved predicates.


\subsection{Sketch of proofs for the propositional case}

We outline the complexity results showing that the satisfiability problem of $\vdash_\PropStandpointLogic$ is NP-complete in a succinct presentation. As for the proofs of soundness and completeness, we only include the theorems and lemmas. The proofs use existing results regarding \kfourfive systems with respect to Kripke models that are serial, transitive and euclidean, and of \sfive with respect to models with equivalence and universal relations, and are extended for standpoint logic following standard methods \cite{Fagin1995ReasoningKnowledge}.

\subsubsection{Soundness and Completeness}

\begin{theorem}[Soundness]
	For every $\phi \in \proplangname$,
	\vspace{0.2em}
	
	\centering $
	\text{if~~} \vdash_{\PropStandpointLogic} \phi
	\hbox{~~then~~}
	\models_{\PropStandpointLogic} \phi \ .
	$
	\vspace{0.2em}
	
	\label{Theorem:soundness}
\end{theorem}

We prove this by induction on the structure of the proof $\tuple{\phi_1,\cdots,\phi_n}$ of $\phi$. In the first place we prove that every instance of an axiom schema is valid.
Then, by considering the truth conditions for formulae of
the forms $\alpha\imp\beta$ and
$\standb{s_{i}}\phi$, it is straightforward that
the rules {\bf MP.} and {\bf RN.} must preserve validity.
Consequently, one can show that all provable formulae are valid, hence that the system is sound.

\begin{theorem}[Completeness]
	%%%%%%%% ATTENTION: WE ARE NOT PUTTING THE PREMISES. VERIFY?
	%Completeness of\/ \ $\vdash_\PropStandpointLogic$:
	%\begin{enumerate}[leftmargin=5em,labelwidth=6em]
	%\item[] $\text{If~~} \modelSo \phi,
	%\text{~~then~~} \vdash_\PropStandpointLogic \phi$ \ .
	%\end{enumerate}
	For every $\phi \in \proplangname$,
	\vspace{0.2em}
	
	\centering
	$ \text{if~~} \models_{\PropStandpointLogic} \phi
	\hbox{~~then~~}
	\vdash_{\PropStandpointLogic} \phi \ .
	$
	\vspace{0.2em}
	
	
	
	\label{Theorem:completeness}
\end{theorem}

The completeness proof follows the lines of \cite{Fagin1995ReasoningKnowledge} for \kdfourfive and \sfive and extends it for \emph{standpoint logic}. The two main building blocks are \emph{Lindenbaum's lemma} \cite{Chellas1980ModalIntroduction}, which states that for a set of formulas $\gamma$, if $\gamma$ is $\PropStandpointLogic$-consistent then we can create a $\PropStandpointLogic$-maximal set of formulas, $\Gamma$, such that $\gamma\subseteq\Gamma$, and the \emph{canonical model}:

\begin{lemma}
	Let $\modelc$ be the canonical model for the system of modal logic $\PropStandpointLogic$, such that \hbox{$\modelc=\tuple{\Precs, \tradaccRelation, \delta}\,$}, in which:
	
	\begin{enumerate}[label=(\alph*), leftmargin=1.5em,labelwidth=2em]
		\item $\Precs$ is the set of all maximal $\PropStandpointLogic$-consistent sets of sentences, such that each $\p{\Gamma}\in\Precs$,
		consists of all formulae that are true at $\p{\Gamma}$.
		\item Each relation $\tradaccrelations\in\tradaccRelation$ is such that $(\p{A},\p{B})\in\tradaccrelations$ iff $\{\phi:\standbs\phi\in A\}\subseteq B$.\label{list:canonical-relation}
		%    \item Each relation $\accrelations\in\accRelation$ can be defined in terms of its homologous $\tradaccrelati
	\end{enumerate}
\end{lemma}

Following a Henkin-style method, we assume that there is some tautology $\models_{\PropStandpointLogic} \psi$ that is not provable $\nvdash_{\PropStandpointLogic} \psi$. Consequently, appending its negation to the theory is consistent, yet we show that for every consistent formula $\phi$ there is a model of the class $\modelclass$ in which $\phi$ is true at at least one precisification. By contradiction, this proves Theorem \ref{Theorem:completeness}. We first show that $\modelc$ models every consistent formula of the language.

\begin{lemma}\label{Lemma:generated-model}
	Let $\modelc$ be the canonical model and $\modelc_{\Gamma}$ be the submodel generated by the non-empty subset $\Precs_{sub}$. Then for each $\pr\in\Precs_{sub}$ and each formula $\phi$, it is the case that $ \ModSat \modelc,\pr||-\phi \text{~~~iff~~~} \ModSat \modelc_{\Gamma},\pr||-\phi$
\end{lemma}

Then, given that $\modelc$ does not belong to $\modelclass$,\textbf{(c)} we show that for any precisification $\p{\Gamma}$ such that $\tuple{\modelc, \p{\Gamma}}\models\phi$, we can create a submodel $\modelc_\Gamma$ that is equivalent to $\modelc$ with respect to $\p{\Gamma}$ and that it is in the class $\modelclass$, where $\star$ is a universal relation and relations can be simplified into sets. Hence, to recapitulate, we show that for any consistent formula $\phi$ there is a model $\modelc_\Gamma$ such that $\tuple{\modelc_\Gamma, \p{\Gamma}}\models\phi$ and $\modelc_\Gamma\in\modelclass$, thereby proving completeness.


\begin{corollary}
	$\PropStandpointLogic$ is a sound and complete axiomatisation with respect to $\modelclass$ for formulas in the language $\proplangname$.
\end{corollary}

% \subsection{Decidability}

% \begin{lemma}\label{Lemma:kripke-model-checking}
% There is an algorithm that, given a finite Kripke structure $\model\finite$
% and a formula $\phi$, determines, in time $O(||\model\finite|| \times |\phi|)$, whether there is a state $\pr$ of $\model\finite$ such that $(\model\finite, \pr) \models \phi$, for $|\phi|$ be the size of $\phi$ and $||\model\finite||$ be the sum of the number of points $\pr$ in $\Precs$ and the number of pairs in the relations $\tradaccrelations\in\tradaccRelation$. I.e. there is an algorithm for checking if $\phi$ is satisfied in $\model\finite$.
% \end{lemma}

% See \cite{Fagin1995ReasoningKnowledge} for a proof of {\bf Lemma \ref{Lemma:kripke-model-checking}}. 
% The strategy to prove the finite model property for $\PropStandpointLogic$ follows closely the proof on \cite{Fagin1995ReasoningKnowledge} and consists in using the result that $\PropStandpointLogic$ is determined by the class of models $\modelclass$ in section \ref{SEC:CH4-soundness-completeness} to show that  $\PropStandpointLogic$ is also determined by the class of $\modelclass\finite$ of finite models, so that 
% $$ 
% \vdash_\PropStandpointLogic \phi 
% \text{~~~~iff~~~~} \modelSo\finite \phi 
% $$

% Soundness is trivial because $\modelclass\finite\subseteq\modelclass$, and hence it remains to show completeness with respect to $\modelclass\finite$. We first show that if a formula is $\PropStandpointLogic$-consistent,
% not only is it satisfiable in some structure (such as the canonical
% structure constructed in the proof of Theorem \ref{Theorem:completeness}), but it is also satisfiable
% in a finite structure  $\model\finite$ in the class $\modelclass$. The proof is
% actually just a variant of the proof of {\bf Theorem \ref{Theorem:completeness} (\emph{Completeness})}.

% Let $Sub^+(\phi)$ be the set consisting of the subformulas of $\phi$ and their negations, that
% is, ${Sub^+(\phi) = Sub(\phi) \cup \{\n\psi\ |\ \psi \in Sub(\phi)\}}$. Let $Con(\phi)$ be the set of maximal
% $\PropStandpointLogic$-consistent subsets of $Sub^+(\phi)$. Theorem \ref{Theorem:Maximal}
% can be used to show that every $\PropStandpointLogic$-consistent subset of $Sub^+(\phi)$ can be extended
% to an element of  $Con(\phi)$. Moreover, a member of  $Con(\phi)$ contains either $\psi$ or $\n\psi$
% for every formula  $\psi\in Sub(\phi)$ (but not both, for otherwise it would not be $\PropStandpointLogic$-consistent), so the cardinality of $Con(\phi)$ is at most  $2^{|Sub(\phi)|}$, which is at most $2^{|\phi|}$,
% since $|Sub(\phi)| \leq |\phi|$.

% We can now construct a structure $\mathcal{M\finite}=\tuple{\Precs\finite,(\accRelation\finite,\preceq),\delta\finite}$ in the class $\modelclass$ identical to the canonical model ({\bf Definition \ref{DEF:canonical-model}}) except that $\Precs = \{ \p{\Gamma}\ |\ \Gamma \in Con(\phi) \}$. Note that the sets in $Con(\phi)$ are $\PropStandpointLogic$-consistent and that the axioms of $\PropStandpointLogic$ guarantee the properties of the relations in $\modelclass$ and hence in $\mathcal{M\finite}$ (as we have proven in section \ref{SEC:CH4-completeness}). Therefore the following restrictions hold for the relations in $(\accRelation\finite,\preceq)$:

% \begin{itemize}
%     \item $\tradaccrelations = \{(\p{\Gamma}\text{, }\ \p{\Sigma})\ |\ \Gamma/\standbs = \Sigma/\standbs\text{, }\ \Gamma/\standbs \subseteq \Sigma\}$
%     \item $\tradaccrelationstar = \{(\p{\Gamma}\text{, }\p{\Sigma})\ |\ \Gamma/\allstandb = \Sigma/\allstandb{, }\ \Gamma/\standbs \subseteq \Gamma{, }\ \Gamma/\standbs \subseteq \Sigma\}$
% \end{itemize}

%  Finally, with a proof identical to that of {\bf Theorem \ref{Theorem:completeness}(a)-(d)}\footnote{See the proof by induction on the structure of $\phi$ with respect to the canonical model}, we can show that for all $\psi\in Sub^+(\phi)$ and $\Gamma\in Con(\phi)$, iff $\psi\in\Gamma$ then $(\mathcal{M\finite},\p{\Gamma})\models\psi$. Hence, $\phi$ is satisfiable in a structure in $\modelclass$ with as many points as the cardinality of $Con(\phi)$, which is at most $2^{|\phi|}$ and, therefore we conclude that the provability problem is decidable.

\subsubsection{Complexity}\label{sec-sub:complexity}
We now show that the satisfiability problem is {\bf NP}-complete. %In this section we partially use the proofs provided in \cite{Fagin1995ReasoningKnowledge,Halpern1992ABelief}

\begin{lemma}
	\label{Theorem:satisfiable-in-phi-states}
	\label{lemma:small-model-property}
	An $\PropStandpointLogic$ formula $\phi$ is satisfiable if and only if it is satisfiable in a structure  $\model^{|\phi|}\in\modelclass$ with at most $|\phi|$ precisifications, for $|\phi|$ be the size\footnote{The size of a formula $\phi$ in $\proplangname$, denoted $|\phi|$,
		is its length over the alphabet $ \mathcal{P} \cup \{\n, \con, (,), \standbi{1}, \dots,\standbi{n}, \allstandb\}$, where $\mathcal{P}$ is the set of atomic formulas.} of the formula $\phi$.
	
	\bigskip
	\begin{proof}
		Let $\model=\tuple{\Precs,\sigma,\delta}$ be a model for $\phi$.
		We obtain a small model $\model'=\tuple{\Precs',\sigma',\delta'}$ as follows.
		In our construction, we often need to randomly pick elements from sets;
		we use the notation $\pick{M}$ to denote a randomly picked element $x\in M$.
		
		For every $s\in\StandConsts$ and subformula $\psi$ of $\phi$, define the set $\Precs^s_\psi$ by structural induction.
		Intuitively, for each subformula of the form $\standbs\psi$ or \mbox{$s'\preceq s$} that is not satisfied in $\M$, the set $\Precs^s_\phi$ randomly picks a witnessing precisification $\pi\in\sigma(s)$.
		\begin{align*}
			\Precs^s_p                   & =\emptyset                              \\
			\Precs^s_{\neg\psi}          & =\Precs^s_{\psi}                        \\
			\Precs^s_{\psi_1\land\psi_2} & =\Precs^s_{\psi_1}\cup\Precs^s_{\psi_2} \\
			\Precs^s_{\standb{s'}\psi}   & =\Precs^s_{\psi}\cup
			\begin{cases}
				\set{\pick{\set{ \pi\in\sigma(s) \guard (\M,\pi)\not\models\psi }}} & \text{ if } s=s' \text{ and } \model\not\models\standbs\psi \\
				\emptyset                                                           & \text{ otherwise}
			\end{cases}                                             \\
			\Precs^s_{s\preceq s'}       & =
			\begin{cases}
				\set{\pick{\sigma(s) \setminus \sigma(s')} } & \text{ if } \M\not\models s\preceq s' \\
				\emptyset                                    & \text{ otherwise}
			\end{cases}
		\end{align*}
		We now define the reduced set of precisifications.
		Then we take all witnesses needed for subformulas of the form $\standbs\psi$ or $s\preceq s'$.
		%;        if $\phi$ contains no such subformulas, we pick an arbitrary precisification from $\sigma(s)$ to guarantee non-emptiness of the resulting $\sigma'(s)$.
		Formally, we define\/:
		\begin{align*}
			\Precs' & = \bigcup_{s\in\S}\Precs^s_\phi
		\end{align*}
		and set, for each $s\in\S$,
		\begin{gather*}
			\sigma'(s) = \sigma(s) \cap \Precs'
		\end{gather*}
		and for each $p\in\PropConsts$,
		\begin{gather*}
			\delta'(p) = \delta(p) \cap \Precs'
		\end{gather*}
		It is easy to see that the size of $\Precs'$ is at most $\card{\Sub(\phi)} + \card{\S}$, as each $\pi\in\Precs'$ is a necessary witness for exactly one subformula of $\phi$.% or was chosen arbitrarily for some $s\in\S$ to satisfy $\sigma'(s)\neq\emptyset$.
		
		We now have to show that $\M'\models\phi$.
		We will show by structural induction that for each subformula $\psi$ of $\phi$ and $\pi\in\Precs'$, we have
		\begin{gather*}
			(\M,\pi)\models\psi \text{ iff } (\M',\pi)\models\psi
		\end{gather*}
		In particular, by the presumption that $\M\models\phi$ this shows that $\M'\models\phi$.
		($\M\models\phi$ implies $(\M,\pi)\models\phi$ for all $\pi\in\Pi$, which implies $(\M,\pi)\models\phi$ for all $\pi\in\Pi'$ by $\Pi'\subseteq\Pi$, which implies $(\M',\pi)\models\phi$ for all $\pi\in\Pi'$ via the below.)
		\begin{description}
			\item[$p$:] $(\M,\pi)\models p$ \\
			iff $\pi\in\delta(p)$\\
			iff $\pi\in\delta(p)\cap\Precs'$ \quad (since $\pi\in\Precs'$) \\
			iff $\pi\in\delta'(p)$\\
			iff $(\M',\pi)\models p$.
			\item[$\neg\psi$:] Exercise.
			\item[$\psi_1\land\psi_2$:] Exercise.
			\item[$\standbs\psi$:]
			\begin{description}
				\item[“if”:]
				We show the contrapositive.
				Let $(\M,\pi)\not\models\standbs\psi$.
				Since $\standbs\psi\in\Sub(\phi)$, there is some $\pi'\in\Precs^s_{\standbs\psi}$ such that $(\M,\pi')\not\models\psi$.
				By definition $\Precs^s_{\standbs\psi}\subseteq\Precs^s_\phi\subseteq\Precs^s\subseteq\sigma'(s)$, whence $\pi'\in\sigma'(s)\subseteq\Precs'$.
				By the induction hypothesis, $(\M',\pi')\not\models\psi$.
				Thus $(\M',\pi)\not\models\standbs\psi$.
				\item[“only if”:]
				Let $(\M,\pi)\models\standbs\psi$.
				Consider an arbitrary $\pi'\in\sigma'(s)$.
				By $\sigma'(s)\subseteq\sigma(s)$, we get $\pi'\in\sigma(s)$.
				Thus $(\M,\pi')\models\psi$ by the presumption.
				Since $\pi'\in\Precs'$, we can invoke the induction hypothesis and obtain $(\M',\pi')\models\psi$.
				Since $\pi'\in\sigma'(s)$ was arbitrarily chosen, also $(\M',\pi)\models\standbs\psi$. \alert{On the other hand, consider $\sigma'(s)=\emptyset$. Then, by the semantics also $(\M',\pi)\models\standbs\psi$}
			\end{description}
			\item[$s'\preceq s$:]
			\begin{description}
				\item[“if”:]
				We show the contrapositive.
				Let $(\M,\pi)\not\models s'\preceq s$.
				Since ${s'\preceq s}\in\Sub(\phi)$, by definition of $\Precs^{s'}$, there is a $\pi'\in\Precs^{s'}$ such that $\pi'\in\sigma(s')\setminus\sigma(s)$.
				Clearly $\pi'\in\Precs^{s'}\subseteq\sigma'(s')$, and $\pi'\notin\sigma(s)$ and $\sigma'(s)\subseteq\sigma(s)$ imply $\pi'\notin\sigma'(s)$.
				Thus $(\M',\pi)\not\models s'\preceq s$.
				\item[“only if”:]
				Let $(\M,\pi)\models s'\preceq s$.
				Then \mbox{$\sigma(s')\subseteq\sigma(s)$}, whence also \mbox{$\sigma(s')\cap\Precs'\subseteq\sigma(s)\cap\Precs'$}, that is, \mbox{$\sigma'(s')\subseteq\sigma'(s)$}.
			\end{description}
		\end{description}
	\end{proof}
\end{lemma}

\begin{theorem}\label{Theorem:np-complete} There is a $NP$-algorithm for deciding whether a formula $\phi$ is $\PropStandpointLogic$-satisfiable. Hence, the satisfiability problem for $\PropStandpointLogic$ is in $NP$.
\end{theorem}

Such an algorithm involves, for a formula $\phi$, nondeterministically guessing a structure $\model\in\modelclass$ with at most $|\phi|$ precisifications and
exactly $|\StandConsts^{\phi}|$ standpoints {\bf (Part 1)}, and deterministically verifying that $\phi$ is satisfied in $\model$  {\bf (Part 2)}.

\noindent{(Part 1).}

The nondeterministic guessing covers (1) deciding the size of $\Precs$, $n\leq |\phi|$, (2) the valuation $\True$ or $\False$ of the primitive propositions $p$ appearing in $\phi$ at every precisification $\p{i\in \{1,\dots, n\}}$, and (3) determining the membership or not of every precisification in each standpoint in $\phi$.
% given a formula $\phi$, we guess a structure $\model=\tuple{\Precs, (\accRelation, \preceq), \delta}$ where (a) $\Precs$ is a set of $n$ precisifications such that $n \leq |\phi|$, (b) $\accRelation$ is a set of $s$ subsets of $\Precs$ such that $s=|\{ i\ |\ \standbi{i}\psi \in Sub(\phi)\}|$ and (c) $\delta(\pr)(p)=\False$ for all $\pr\in\Precs$ and all primitive propositions not appearing in $\phi$. 
% Consequently, the nondeterministic guessing involves (1) deciding the size of $\Precs$, $n$, (2) the valuation $\True$ or $\False$ of the primitive propositions $p$ appearing in $\phi$ at every point $\p{i\in \{1,\dots, n\}}$, and (3) the membership or not of every point in each standpoint in $\phi$, i.e $\forall\p{i}\in\Precs,\ \forall\accrelation{j}\in\accRelation\ \{    \p{i}\in\accrelation{j} \dis \p{i}\notin\accrelation{j}\}$. 
The number of atomic propositions $p^\phi$ to guess (2), plus the number of distinct modal standpoint operators $s^\phi$ to guess (3) is less than the size of $\phi$. Therefore, given that $(p^\phi+s^\phi)\leq m$, and there is $n \leq m$ precisifications, the structure can be guessed at $O(m^2)$ time.

\noindent{(Part 2).}

We now verify that there is a $\pr$ such that $(\model,\pr)\models\phi$.% We know by {\bf Lemma \ref{Lemma:kripke-model-checking}} that this can be done in time $O(||\model|| \times |\phi|)$, for $||\model\finite||$ the sum of the number of points $\pr$ in $\Precs$ and the number of pairs in the relations $\tradaccrelations\in\tradaccRelation$. In the worst case we have $n\times n$ relations in each $\tradaccrelations$ and we have at most $s<m$ relations or standpoints. Consequently we know that we can verify it deterministically in at least $O(m^3)$ time.

%Moreover, we can show that, because of the particularities of the models in $\modelclass$, we can check whether $\phi$ is satisfied at some state $\pr\in\Precs$ in time $O(m^2)$ (see {\bf Lemma \ref{Theorem:standpoint-model-checking}} below). 

\begin{lemma} \label{Theorem:standpoint-model-checking}
	There is an algorithm that, given a finite Kripke structure $\model$ of the class $\modelclass$ and a formula $\phi$, determines, in time $O(|\phi|^2)$, whether $(\model, \pr) \models \phi$ for some precisification $\pr$ of $\model$, for $|\phi|$ both the size of $\phi$ and the upper bound of  $|S|$.
\end{lemma}


\begin{proof}
	
	%Let $Sub(\phi)=\{\phi_1, \dots, \phi_m\}$ be the set of subformulas of $\phi$, listed in order of length and with ties broken arbitrarily. Thus we have $\phi_m=\phi$, and if $\phi_i$ is a subformula of $\phi_j$ , then $i < j$.
	%There are at most $|\phi|$ subformulas of $\phi$ ({\bf Definition \ref{DEF:subformulas}}), so we must have $m \leq |\phi|$.
	
	We label each precisification $\pr$ in $\model$ with $\phi_j$ or $\n\phi_j$ depending on whether $(\model,\pr)\models\phi_j$, and the model $\model$ with $\standbs\phi_j$ or $\n\standbs\phi_j$ depending on whether $(\model)\models\standbs\phi_j$ (for all precisifications). %Given that there are $m$ subformulas and at most $m$ states, we are at least at complexity $O(m^2)$. Now, let us see a sketch of the algorithm.
	\vspace{0.5em}
	
	\noindent\textbf{Algorithm (1): }Let us take the subformulas of $\phi$ by order. For each subformula $\phi_j\in Sub(\phi)$, if $\phi_j$ is:
	\begin{itemize}
		\item An atomic proposition $p$: for each $\pr\in\Precs$ we check if $(\model,\pr)\models p$ and we label $\pr$ with $p$ (or $\n p$).  \hfill ($O(m)$)
		\item A formula of the form $\n\phi_i$ or $\phi_i\con\phi_h$: for each  $\pr\in\Precs$ we check if either $\pr$ or $\model$ is labelled with $\n\phi_i$ or both $\phi_i$ and $\n\phi_h$ respectively and label accordingly.\hfill  ($O(m)$)
		
		\item A formula of the form $\st\preceq\sp$: we check if $\accrelations\subseteq\accrelation{\sp}$. Then, we label $\model$ accordingly. \hfill ($O(\size{S}^2)$)
		
		\item A formula of the form $\standbs\phi_i$: we check if all $\pr\in\accrelations$ are labelled with $\phi_i$. Then, we label $\model$ (with $\standbs\phi_i$ or $\n\standbs\phi_i$) accordingly. \hfill ($O(2m) => O(m)$)
	\end{itemize}
	
	% (Note that checking $\standbs\phi$ formulae is more efficient than one might expect because
	% although they depend on all precisifications within the set associated with standpoint $s$,
	% the value of $\standbs\phi$ must be the same at all precisifications, so only has to
	% be computed once.)
	
	
	Given that the size of $Sub(\phi)$ is at most $m$, we can easily see that the algorithm has a complexity $O(m^2)$. This is because formulas of the kind $\standbs\phi_i$ have the same valuation for all precisifications in the models $\modelclass$.
\end{proof}

\begin{corollary}
	By Theorem \ref{Theorem:satisfiable-in-phi-states}, if $\phi$ is satisfiable then it will be satisfied by one of the models created in this way. If $\phi$ is not satisfiable no guess will be right. Thus, we have a nondeterministic $O(m^2)$ algorithm for deciding if $\phi$ is satisfiable.
\end{corollary}


\subsection{Translation for Propositional Standpoint Logic}


Consider a formula $\phi$ of propositional standpoint logic.
We assum the vocabulary $\tuple{\PropConsts,\StandConsts}$ to be implicitly given through $\phi$, that is, as collecting all propositional and standpoint constants occurring in $\phi$.
Define the \emph{size} of $\phi$, written $\size{\phi}$, as the number of its subformulas (it is easy to define via structural induction).
Clearly, then, $\card{\PropConsts}+\card{\StandConsts}\leq\size{\phi}$.
In what follows, we will typically denote \mbox{$m=\size{\phi}$} and assume that the standpoint symbol $\star$ occurs in $\phi$ (this is w.l.o.g.\ as any $\phi$ is equivalent to $\standb{\star}\phi$).

The translation to be defined will make explicit use of precisifications of the form $\pi_\psi$ for subformulas $\psi$ of $\phi$.
In words, there is exactly one precisification symbol for each subformula of $\phi$.
While not all of these might be relevant in every case, the small model property guarantees that by allowing for this number of precisifications, we do not exclude potential models.
Formally, denote by
\begin{gather*}
	\Pi_\phi = \set{ \pi_\psi \guard \psi\in\Sub(\phi) }
\end{gather*}
the set of all such standpoint symbols.

We will translate $\phi$ into a formula of (standpoint-free) propositional logic over the following vocabulary (keeping in mind that we wish to emulate models $\tuple{\Pi,\sigma,\delta}$ (more precisely, models $\tuple{\Pi_\phi, \sigma, \delta}$) of standpoint logic with valuations over these atoms)\/:
\begin{itemize}
	\item atoms of the form $p_\pi$ for original propositional atoms \mbox{$p\in\PropConsts$} and $\pi\in\Pi_\phi$ (intuitively expressing that $\pi\in\delta(p)$),
	\item atoms of the form $s_\pi$ for standpoint constants \mbox{$s\in\StandConsts$} and $\pi\in\Pi_\phi$ (intuitively expressing that $\pi\in\sigma(s)$).
\end{itemize}
(Since ${\star}\in\S$, there are also atoms of the form $\star_{\pi}$ for $\pi\in\Pi_\phi$.)
We denote the resulting propositional vocabulary by \mbox{$\Pphi=\set{ p_\pi, s_\pi \guard p\in\PropConsts, s\in\StandConsts, \pi\in\Pi_\phi }$}.

The top-level translation is then defined to set\/:
\begin{align*}
	\Trans(\phi)                   & = \bigland_{\pi\in\Pi_\phi}\trans(\pi,\phi) \land \bigland_{\pi\in\Pi_\phi}{\star}_{\pi} \\% \land \bigland_{s\in\S}\biglor_{\pi\in\Pi_\phi}s_{\pi} \\
	\intertext{where, by structural induction,}
	\trans(\pi, p)                 & = p_\pi                                                                                  \\
	\trans(\pi, \lnot\psi)         & =\lnot\trans(\pi,\psi)                                                                   \\
	\trans(\pi, \psi_1\land\psi_2) & = \trans(\pi,\psi_1)\land\trans(\pi,\psi_2)                                              \\
	\trans(\pi', \standbs\psi)     & = \bigland_{\pi\in\Pi_\phi}\left(s_\pi\limplies\trans(\pi,\psi)\right)                   \\
	\trans(\pi', s'\preceq s)      & = \bigland_{\pi\in\Pi_\phi}\left(s'_\pi\limplies s_\pi\right)
\end{align*}

The main translation $\Trans$\/:
(1) asserts that the given formula $\phi$ must hold in all precisifications,
(2) asserts that $\sigma(\star)=\Pi_\phi$ in any valuation of the resulting vocabulary.
%,(3) asserts that all standpoints are non-empty, i.e.\ contain at least one precisification.

The $\trans$ part of the definition just emulates universal quantification over precisifications via conjunction, and emulates the single first-order variable via keeping track of the relevant precisification explicitly.
This naive version of the translation (in case of subformulae of the form $\standbs\psi$) still creates a conjunction of size \mbox{$\card{\Pi_\phi}=\size{\phi}$} for each level of nesting of standpoint modalities;
for a $\phi$ of depth $d$, the resulting $\Trans(\phi)$ could be of size up to $\size{\phi}^d$.
This can be avoided by providing a formula in \emph{standpoint standard normal form}, for which transformations are provided later in this document.

Given a valuation \mbox{$v:\Pphi\to\set{\True,\False}$} of the resulting propositional vocabulary, the associated interpretation \mbox{$\M_v=\tuple{\Pi_\phi,\sigma,\delta}$} is clear:
\begin{itemize}
	\item     \mbox{$\sigma(s)=\set{\pi\in\Pi_\phi\guard v(s_\pi)=\True }$}, $s\in\StandConsts$,
	\item     \mbox{$\delta(p)=\set{\pi\in\Pi_\phi\guard v(p_\pi)=\True }$}, $p\in\PropConsts$.
\end{itemize}
In the opposite direction (i.e., given an arbitrary $\M=\tuple{\Pi,\sigma,\delta}$), the transformation is not as immediate as we have no guarantees on the size and contents of $\Pi$.
A start is the result on the small model property of propositional standpoint logic, which basically guarantees that models are not only of a convenient size, but can always be brought into a specific form – namely using exactly the set of precisifications $\Pi_\phi$ we used in the translation.

\begin{lemma}
	Any satisfiable formula $\phi$ of propositional standpoint logic has a model over precisification set $\Pi_\phi$.
	
	\bigskip
	\begin{proof}
		We will show that if $\phi$ has a model \mbox{$\M=\tuple{\Pi,\sigma,\delta}$}, then it also has a model \mbox{$\M'=\tuple{\Pi_\phi,\sigma',\delta'}$}.
		By \ref{lemma:small-model-property}, we can assume w.l.o.g.\ that $\M$ is a minimal model.
		Our main task in this proof is to identify the relevant witnessing precisifications in $\Pi$ and map them to $\Pi_\phi$ (adjusting $\sigma$ and $\delta$ accordingly).
		To do that, we define a relation ${\sim}\subseteq\Pi\times\Pi_\phi$ and then use structural induction to show that for any subformula $\psi$ of $\phi$ and any $\pi\sim\pi'$, we have
		\begin{gather}
			\label{dagger}
			\M,\pi\models\psi \text{ iff } \M',\pi'\models\psi
		\end{gather}
		The relation $\sim$ is now a $\subseteq$-minimal subset of $\Pi\times\Pi_\phi$ such that\/:
		\begin{itemize}
			\item $\pi\sim\pi_{\standbs\psi}$ whenever $(\M,\pi)\not\models\psi$;
			\item $\pi\sim\pi_{s'\preceq s}$ whenever $\pi\in\sigma(s')\setminus\sigma(s)$;
			%\item for every $s\in\S$\/:
			%   \begin{itemize}
			%    \item there is a $\pi\in\Pi$,
			% \item and a $\psi\in\Sub(\phi)\setminus\set{s'\preceq s\in\Sub(\phi)\guard s'\in\S}$,
			%   \item such that $\pi\sim\pi_{\psi}$.
			%\end{itemize}
		\end{itemize}
		
		Accordingly, we define $\delta'$ and $\sigma'$\/:
		\begin{enumerate}
			\item for $p\in\PropConsts$, we set $\delta'(p)=\set{ \pi'\in\Pi_\phi \guard \pi\in\delta(p), \pi\sim\pi' }$,
			\item for $s\in\S$, we set $\sigma'(s)=\set{ \pi'\in\Pi_\phi \guard \pi\in\sigma(s), \pi\sim\pi' }$.
		\end{enumerate}
		
		Now for proving \Cref{dagger}; let $\psi\in\Sub(\phi)$ and $\pi\sim\pi'$.
		\begin{description}
			\item[$p$:] $\M,\pi\models p$\\
			iff $\pi\in\delta(p)$\\
			iff $\pi\in\delta(p)$ and $\pi\sim\pi'$\\
			iff $\pi'\in\delta'(p)$\\
			iff $(\M',\pi')\models p$.
			\item[$\neg\psi$:] Exercise.
			\item[$\psi_1\land\psi_2$:] Exercise.
			\item[$\standbs\psi$:]
			\begin{description}
				\item[“if”:]
				We show the contrapositive.
				Let $(\M,\pi)\not\models\standbs\psi$.
				Then there is a $\pi''\in\sigma(s)$ such that $(\M,\pi'')\not\models\psi$.
				By definition of ${\sim}$, we have $\pi''\sim\pi_{\standbs\psi}$.
				Invoking the induction hypothesis, we obtain $(\M',\pi_{\standbs\psi})\not\models\psi$.
				Furthermore, $\pi_{\standbs\psi}\in\sigma'(s)$ by definition of $\sigma'$.
				In combination, $(\M',\pi_{\standbs\psi})\not\models\standbs\psi$.
				\item[“only if”:]
				Let $(\M,\pi)\models\standbs\psi$.
				Let $\pi''\in\sigma'(s)$ be arbitrary.
				Then the corresponding $\pi'''\sim\pi''$ satisfies $\pi'''\in\sigma(s)$ by definition.
				Thus $(\M,\pi''')\models\psi$.
				By the induction hypothesis, we obtain $(\M',\pi'')\models\psi$.
				Since $\pi''$ was arbitrarily chosen, we get $(\M',\pi')\models\standbs\psi$.  \alert{On the other hand, consider $\sigma'(s)=\emptyset$. Then, by the semantics also $(\M',\pi)\models\standbs\psi$}
			\end{description}
			\item[$s'\preceq s$:]
			\begin{description}
				\item[“if”:]
				We show the contrapositive.
				Let $(\M,\pi)\not\models s'\preceq s$.
				Then there is a $\pi''\in\sigma(s')\setminus\sigma(s)$.
				By definition, we get $\pi''\sim\pi_{s'\preceq s}$.
				By $\pi''\in\sigma(s')$ and $\pi''\sim\pi_{s'\preceq s}$, according to the definition of $\sigma'$ we get $\pi_{s'\preceq s}\in\sigma'(s')$.
				By definition of ${\sim}$, for all $\pi'''\in\Pi$, whenever $\pi'''\sim\pi_{s'\preceq s}$ then $\pi'''\notin\sigma(s)$.
				Thus $\pi_{s'\preceq s}\notin\sigma'(s)$.
				In combination, we get $(\M',\pi')\not\models s'\preceq s$.
				\item[“only if”:]
				Let $(\M,\pi)\models s'\preceq s$.
				Then $\sigma(s')\subseteq\sigma(s)$.
				Let $\pi''\in\sigma'(s')$ be arbitrary.
				By definition of $\sigma'$, there is a $\pi'''\in\sigma(s')$ with $\pi'''\sim\pi''$.
				Due to $\sigma(s')\subseteq\sigma(s)$ we get $\pi'''\in\sigma(s)$.
				By definition of $\sigma'$, we have $\pi''\in\sigma'(s)$.
				Since $\pi''$ was arbitrarily chosen, we get $\sigma'(s')\subseteq\sigma'(s)$ and thus $(\M',\pi')\models s'\preceq s$.
			\end{description}
		\end{description}
	\end{proof}
\end{lemma}

We call any model of $\phi$ that is of the form $\tuple{\Pi_\phi,\sigma,\delta}$ a \emph{standard model}.
When concerned with satisfiability in what follows, we will be able to restrict our attention to standard models.
The main benefit of this is that embedding standard models into the propositional language of $\Trans(\phi)$ very easily.
We embed as follows\/:
\begin{itemize}
	\item For each standpoint constant $s\in\S$ and precisification symbol $\pi\in\Pi_\phi$, we set \mbox{$v_\M(s_{\pi})=\True$} iff \mbox{$\pi\in\sigma(s)$};
	\item for each (original) propositional atom \mbox{$p\in\PropConsts$} and precisification symbol $\pi\in\Pi_\phi$, we set \mbox{$v_\M(p_{\pi})=\True$} iff \mbox{$\pi\in\delta(p)$};
	\item for each precisification symbol $\pi\in\Pi_\phi$, we set \mbox{$v_\M({\star}_{\pi})=\True$}.
\end{itemize}

These mappings pave the way for showing soundness and completeness (i.e.\ correctness) of the proposed translation.

\begin{lemma}
	Let $\phi$ be a formula of propositional standpoint logic over vocabulary $\tuple{\PropConsts,\StandConsts}$,
	\mbox{$\M=\tuple{\Pi_\phi,\sigma,\delta}$} be a standard interpretation for $\tuple{\PropConsts,\StandConsts}$ (with respect to $\phi$),
	and \mbox{$v:\Pphi\to\set{\True,\False}$} be a propositional interpretation for $\Pphi$.
	Furthermore, assume that\/:
	\begin{enumerate}
		\item For each $s\in\StandConsts$ and $\pi\in\Pi_\phi$, we have $v(s_\pi)=\True$ iff $\pi\in\sigma(s)$;
		\item for each $p\in\PropConsts$ and $\pi\in\Pi_\phi$, we have $v(p_\pi)=\True$ iff $\pi\in\delta(p)$.
	\end{enumerate}
	For any $\pi\in\Pi_\phi$ and subformula $\psi$ of $\phi$, we find that
	\begin{gather*}
		\M,\pi\models\psi \text{ iff } v(\trans(\pi,\psi))=\True
	\end{gather*}
	\begin{proof}
		We use structural induction on $\psi$.
		\begin{description}
			\item[$\psi=p$:] $\M,\pi\models p$ iff $\pi\in\delta(p)$ iff $v(p_\pi)=\True$ iff $v(\trans(\pi,p))=\True$.
			\item[$\psi=\neg\xi$:] Exercise.
			\item[$\psi=\xi_1\land\xi_2$:] Exercise.
			\item[$\psi=\standbs\xi$:] $\M,\pi\models\standbs\xi$\\
			iff for all $\pi'\in\sigma(s)$, $\M,\pi'\models\xi$\\
			iff (IH) for all $\pi'\in\sigma(s)$, $v(\trans(\pi',\xi))=\True$\\
			iff for all $\pi'\in\Pi_\phi$, if $\pi'\in\sigma(s)$, then $v(\trans(\pi',\xi))=\True$\\
			iff for all $\pi'\in\Pi_\phi$, if $v(s_{\pi'})=\True$, then $v(\trans(\pi', \xi))=\True$\\
			iff for all $\pi'\in\Pi_\phi$, $v(s_{\pi'}\limplies\trans(\pi',\xi))=\True$\\
			iff $v(\bigland_{\pi'\in\Pi_\phi}(s_{\pi'}\limplies\trans(\pi',\xi))=\True$\\
			iff $v(\trans(\standbs\xi))=\True$.
			\item[$\psi=s'\preceq s$:] $\M,\pi\models s'\preceq s$\\
			iff $\sigma(s')\subseteq\sigma(s)$\\
			iff for all $\pi'\in\Pi_\phi$, if $\pi'\in\sigma(s')$, then $\pi'\in\sigma(s)$\\
			iff for all $\pi'\in\Pi_\phi$, if $v(s'_{\pi'})=\True$, then $v(s_{\pi'})=\True$\\
			iff for all $\pi'\in\Pi_\phi$, $v(s'_{\pi'}\limplies s_{\pi'})=\True$\\
			iff $v(\bigland_{\pi'\in\Pi_\phi}(s'_{\pi'}\limplies s_{\pi'}))=\True$\\
			iff $v(\trans(\pi, s'\preceq s))$.
		\end{description}
	\end{proof}
\end{lemma}

Using this lemma, it should now be possible to show correctness.

\begin{theorem}
	A formula $\phi$ is satisfiable in propositional standpoint logic if and only if the formula $\Trans(\phi)$ is satisfiable in propositional logic.
	
	\bigskip
	\begin{proof}
		\begin{description}
			\item[“if” (Soundness):]
			Let $v:\Pphi\to\set{\True,\False}$ be such that $v(\Trans(\phi))=\True$.
			We use the interpretation $\M_v$ defined before and show that $\M_v\models\phi$.
			It is instructive to note that $\M_v$ is indeed a model of standpoint logic, as $\sigma(\star)=\Pi_\phi$ by the second conjunct. %, and $\sigma(s)\neq\emptyset$ for each $s\in\StandConsts$ by the third conjunct.
			Since $\M_v\models\phi$ iff $\M_v,\pi\models\phi$ for all $\pi\in\Pi_\phi$, we show the latter.
			Consider any $\pi\in\Pi_\phi$.
			Clearly $v(\trans(\pi,\phi))=\True$ by assumption.
			By the lemma above, $\M,\pi\models\phi$.
			\item[“only if” (Completeness):]
			Let $\M=\tuple{\Pi_\phi,\sigma,\delta}$ be a standard model of $\phi$, that is, \mbox{$\M\models\phi$}.
			We have to show that $\Trans(\phi)$ is satisfiable.
			We use the propositional valuation $v_\M$ defined above and show that $v_\M(\Trans(\phi))=\True$.
			\begin{enumerate}
				\item $\bigland_{\pi\in\Pi_\phi}\trans(\pi,\phi)$:
				By presumption, \mbox{$\M\models\phi$}, that is, \mbox{$\M,\pi\models\phi$} for each \mbox{$\pi\in\Pi_\phi$}.
				By the lemma above, in each such case we get that \mbox{$v_\M(\trans(\pi,\phi))=\True$}.
				Overall, it follows that \mbox{$v_\M(\bigland_{\pi\in\Pi_\phi}\trans(\pi,\phi))=\True$}.
				\item $\bigland{\star}_{\pi}$: By definition, $v_\M({\star}_{\pi})=\True$ for any $\pi\in\Pi_\phi$.
				%  \item $\bigland_{s\in\S}\biglor_{\pi\in\Pi_\phi}s_{\pi}$:
				%     Since $\M$ is a model of $\phi$ in standpoint logic, for each \mbox{$s\in\S$} we find that \mbox{$\sigma(s)\neq\emptyset$}, that is, \mbox{$\sigma(s)\cap\Pi_\phi\neq\emptyset$}, that is, there is some \mbox{$\pi\in\Pi_\phi$} such that \mbox{$\pi\in\sigma(s)$}.
				%    By definition of $v_\M$, the claim follows.
			\end{enumerate}
		\end{description}
	\end{proof}
\end{theorem}
\iffalse
\subsection{Normal Form for Propositional Standpoint Logic}

We provide a normal form in which all formulas in $\proplangname$ can be expressed. Several normal forms have been proposed for modal logics in general, and for multi-agent modal logics in particular. For instance, a disjunctive normal form is defined in \cite{Bienvenu2010KnowledgeS5} for a (single-agent) modal logic satisfying \sfive. Moreover, the prime implicate normal forms (PINFs) \cite{Bienvenu2008PrimeConcepts.} have been proposed for the description logic $ALC$, which is a syntactic variant of a multi-agent modal logic {\bf K}, and the cover disjunctive normal forms (CDNFs) \cite{Cate2006DefinitoriallyLogics.} support single-modal logics \kdfourfive and \sfive as shown in \cite{Hales2011RefinementKnowledge} and have been extended for a multi-agent modal logic \kdfourfive in \cite{Hales2012RefinementAgents}.

In what follows, we %extend the single-agent CDNFs in \cite{Hales2011RefinementKnowledge} to the standpoint modalities, and we name the extension \emph{Standpoint Prenex Normal Form}. For this purpose we will first 
introduce a generalisation of the prenex normal form to the multiple modalities of standpoint logic. As expected, formulae in standpoint prenex normal form do not have nested modal operators.

\begin{definition}[Standpoint prenex normal form]
	A formula in standpoint prenex normal form is specified by the following abstract syntax:
	$$\alpha = \  \delta \ \ \text{ or }\ \
	\alpha =(\alpha' \dis \alpha'')$$
	
	\noindent That is, a formula $\alpha$ is either a disjunction of formulas $\alpha' \dis \alpha''$ or a term $\delta$ such that:
	$$
	\delta =  r\ \
	\text{ or }\ \
	\delta =  s\ \
	\text{ or }\ \
	\delta = \standbs r\ \
	\text{ or }\ \
	\delta = \standds r\ \
	\text{ or }\ \
	\delta = (\delta' \con \delta'')$$
	
	\noindent where $r$ is a propositional formula and $s$ is a sharpening statement or its negation.
\end{definition}

%\theoremstyle{plain}
\begin{theorem}\label{lemma:standpoint-prenex}
	Every formula in $\PropStandpointLogic$ is equivalent to a formula in standpoint prenex normal form.
\end{theorem}

\begin{lemma}\label{lemma:normal-form-equivalences}
	We have the following equivalences in $\PropStandpointLogic$:
	\begin{enumerate}
		\item $\standbs (\phi \dis (\psi \con \standbsp \beta) ) \dimp
		(\standbs(\phi \dis \psi ) \con \standbsp \beta)\dis
		(\standbs\phi \con \n\standbsp \beta) )$
		\item $\standbs (\phi \dis (\psi \con \standdsp \beta) ) \dimp
		(\standbs(\phi \dis \psi ) \con \standdsp \beta)\dis
		(\standbs\phi \con \n\standdsp \beta) )$
		\item $\standbs (\sp \preceq s'' ) \dimp (\sp \preceq s'' )$
	\end{enumerate}
	
	\bigskip
	
	\begin{proof}
		(1) and (2) are proven in \cite{Meyer2004EpistemicScience} for every formula in a logic \sfive with a single modality (hence $\st$ and $\sp$ are the same) and extended to \kdfourfive in \cite{Hales2012RefinementAgents}. It is easy to see that with the stronger standpoint interaction axioms \asfour and \asfive instead of {\bf 4} and {\bf 5}, the exact same proof holds for $\PropStandpointLogic$.
		
		% Specifically, for (1): We show that for any ///// TODO
		
		(3) We prove by semantical argument that for any standpoint model $\model$ and precisification $\pr$, $(\model,\pr)\models \standbs (\sp \preceq s'' ) \leftrightarrow (\sp \preceq s'' )$.
		First, assume that $ (\model,\pr)\models  \standbs (\sp \preceq s'' )$. Then, given that the standpoint $\st$ is non empty, there must be at least one precisification $\pp$ such that $\pp\in\sigma(s)$ and such that $(\model,\pp)\models (\sp \preceq s'')$. By the semantics, if this is the case in one precisification, then it must be the case in all precisifications, and thus also in $\pr$.
		In the opposite case, if $ (\model,\pr)\models \neg \standbs (\sp \preceq s'' )$. Then, there must be a precisification $\pp$ such that $ (\model,\pp)\models \neg (\sp \preceq s'' )$. Again by the semantics this implies that also for $\pr$ it is the case that $ (\model,\pr)\models \neg (\sp \preceq s'' )$.
	\end{proof}
	
\end{lemma}



\begin{proof}[Proof of Theorem \ref{lemma:standpoint-prenex}]
	A proof that every formula in \sfive is equivalent to a formula in prenex normal form is provided in  \cite{Meyer2004EpistemicScience}. Such a proof applies also to the case of a \kdfourfive single modal logic, as shown in \cite{Hales2011RefinementKnowledge}, and also to \emph{standpoint logic} following {\bf Lemma \ref{lemma:normal-form-equivalences}} and the multi-modal theorems $\;\proveSo\!\standbsp\!\standbs\phi\!\imp\!\standbs\phi\;$ and $\;\proveSo\!\standbsp\!\n\standbs\phi\!\imp\!\n\standbs\phi\;$ instead of $\;\vdash\!\Box\!\Box\phi\!\imp\!\Box\phi\;$ and $\;\vdash\!\Box\!\n\Box\phi\!\imp\!\n\Box\phi\;$.
\end{proof}
\fi
\subsubsection{Translation from Standpoint Standard Normal Form}

We use the previous translation \todo{In an implementation we could limit the number of precisifications to $|\mathcal{S}|+|\{\p{\phi} | \standd \phi\in Sub(\phi)\}|$ and adapt the small model property proof so they fit well together?} and we show that the size of $trans(\phi)$ is polinomial with respect to $|\phi|$ if $\phi$ is a formula in Standpoint Propositional Normal Form.

\vspace{1em}

\begin{proof}
	
	Consider a formula $\phi$ of size $|\phi|$. For the translation we define $\Pi_\phi = \set{ \pi_\psi \guard \psi\in\Sub(\phi) }$ and thus $|\Pi_\phi| \leq |\phi|$.
	
	It is then easy to see that the size of the formula $Trans(\phi)$ is the summation of the sizes of its two main conjunct plus the conjunction connective.
	
	For all $\pr$, $|trans(\pr,\phi)|$ is clearly cuadratic in the size of $\phi$ because the standpoint standard normal form guarantees that no nested modalities occur and that standpoint assertions are not preceded by modal operators in $\phi$.  Consequently, the rules that introduce quantification over the precisifications (i.e. $\trans(\pi', \standbs\psi)  = \bigland_{\pi\in\Pi_\phi}\left(s_\pi\limplies\trans(\pi,\psi)\right)$ and $\trans(\pi', s'\preceq s) = \bigland_{\pi\in\Pi_\phi}\left(s'_\pi\limplies s_\pi\right)$) also do not nest.
	
	As this applies to all precisifications in $\Pi_\phi$, $|\bigland_{\pi\in\Pi_\phi} trans(\pr,\phi)|$ is cubic on the size of $\phi$, and $|\bigland_{\pi\in\Pi_\phi}{\star}_{\pi}|$ is clearly linear on $|\phi|$.
	
\end{proof}


%
%
%\begin{definition}[Prenex size]
%	The prenex size of a formula $\alpha$ in standpoint prenex normal form is defined as follows:
%	
%	$$ps(\alpha) =  | \{ \ \ t  \ \  |  \ \   \alpha = \  \delta \text{ or } \alpha =(\alpha' \dis \alpha'') , $$
%	$$	\delta =  r  
%	\text{ or } 
%	\delta =  s  
%	\text{ or } 
%	\delta = \standbs r
%	\text{ or }
%	\delta = \standds r
%	\text{ or }
%	\delta = (\delta' \con \delta''), $$ 
%	$$ t = r  \text{ or } t = s \} | $$
%	
%	\noindent where $r$ is a propositional formula and $s$ is a sharpening statement or its negation.
%	
%\end{definition}

